Best of Both Worlds Guarantees for Equitable Allocations

Equitability is a well-studied fairness notion in fair division, where an allocation is equitable if all agents receive equal utility from their allocation. For indivisible items, an exactly equitable allocation may not exist, and a natural relaxation is EQ1, which stipulates that any inequitability should be resolved by the removal of a single item. In this paper, we study equitability in the context of randomized allocations. Specifically, we aim to achieve equitability in expectation (ex ante EQ) and require that each deterministic outcome in the support satisfies ex post EQ1. Such an allocation is commonly known as a `Best of Both Worlds' allocation, and has been studied, e.g., for envy-freeness and MMS. We characterize the existence of such allocations using a geometric condition on linear combinations of EQ1 allocations, and use this to give comprehensive results on both existence and computation. For two agents, we show that ex ante EQ and ex post EQ1 allocations always exist and can be computed in polynomial time. For three or more agents, however, such allocations may not exist. We prove that deciding existence of such allocations is strongly NP-complete in general, and weakly NP-complete even for three agents. We also present a pseudo-polynomial time algorithm for a constant number of agents. We show that when agents have binary valuations, best of both worlds allocations that additionally satisfy welfare guarantees exist and are efficiently computable.

==> figures/2agent-iBiased.tex <==
% \begin{algorithm}
%     \caption{An $i$-Biased \EQ{1} Allocation for Two Agents}\label{alg:biasedtwoagents} 
%     % \hspace*{\algorithmicindent} \textbf{Input}: $\mathcal{I}: \langle [2], [m], \{v_i\}_{i \in [n]} \rangle$ and the \EQ{x} allocation $A$ obtained from the greedy algorithm.\\ 
%     % \hspace*{\algorithmicindent} \textbf{Output:} An $i$-Biased \EQ{1} Allocation $A'$
%     \begin{algorithmic}[1]
%         \State Initialize: $A_1' \leftarrow A_1 \cup \{g\}$ and $A_2' \leftarrow A_2 \setminus \{g\}$ for some $g \in A_2$
%         \For {$s\in C$}
%         \If {$v_1(A_1\setminus\{s\}) \geq v_2(A_2'\cup s)$}
%         \State $A_1' \leftarrow A_1' \setminus \{s\}$,
%         \State  $A_2' \leftarrow A_2' \cup \{s\}$ 
%         \Else
%         \State Break
%         \EndIf
%         \EndFor
%         \Return $A'$
%     \end{algorithmic}
% \end{algorithm}




==> figures/algo_biasedbinary.tex <==

\begin{algorithm}
    \caption{An $i$-Biased \EQ{1} Allocation for Binary Valuations}\label{alg:biasedbinary} 
    \hspace*{\algorithmicindent} \textbf{Input}: $\mathcal{I}: \langle [n], [m], \{v_i\}_{i \in [n]} \rangle$ and an \EQ{1} allocation $A$ \\ 
    \hspace*{\algorithmicindent} \textbf{Output:} An $i$-Biased \EQ{1} Allocation $A'$
    \begin{algorithmic}[1]
        \State Let $R$ be the set of rich agents under $A$
        \If {$v_i\{g\} = 1$ for some $\{g \in A_r: r \in R\}$}
        \State $A_i' \leftarrow A_i \cup \{g\}$,
        \State  $A_r' \leftarrow A_r \setminus \{g\}$ 
        \State  $A_j' \leftarrow A_j ~\forall~ j \in [n] \setminus \{i \cup r\}$
        \Else 
        \State $A_i' \leftarrow A_i$
        \For {$r \in R$}
        \State Let $g \in A_r$ be such that $v_r(g) =1 $
        \State $A_r' \leftarrow A_r \setminus \{g\}$
        \State $A_i' \leftarrow A_i' \cup \{g\}$
        \EndFor
        \State $A_j' \leftarrow A_j ~\forall~j \in [n] \setminus  \{i \cup R\}$
        \EndIf
        \Return $A'$
    \end{algorithmic}
\end{algorithm}


==> figures/strong_npc.tex <==
\begin{figure}[h]
    \centering
    \renewcommand{\arraystretch}{1.3} % Increase line spacing
    \begin{tabular}{c|ccccccc}
        % \toprule
          & $g_1$ & $g_2$     & $\ldots$ & $g_{m-1}$ & $g_m$ & $d_1$ & $d_2$ \\
          \hline
    $a_0$ & $\frac{2m}{3}T$   & $\frac{2m}{3}T$     & $\ldots$ &  $\frac{2m}{3}T$ & $\frac{2m}{3}T$ & $T$ & $\left(\frac{m}{3}-1\right)T$ \\
    $a_1$ & $b_1$  & $b_2$   & $\ldots$ & $b_{m-1}$ & $b_m$ & $\frac{m^2}{3}T$ & $\frac{m^2}{3}T$    \\
    $a_2$ & $b_1$  & $b_2$  & $\ldots$ & $b_{m-1}$ & $b_m$ & $\frac{m^2}{3}T$ & $\frac{m^2}{3}T$    \\
    $\vdots$ & $\vdots$ & $\vdots$ & $\ddots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ \\
    $a_k$ & $b_1$  & $b_2$  & $\ldots$ & $b_{m-1}$ & $b_m$ & $\frac{m^2}{3}T$ & $\frac{m^2}{3}T$ \\
    % \bottomrule    
    \end{tabular}
    \caption{\centering Reduction for the proof of \Cref{thm:strong_NPC}.}
    \label{tab:table_reduction_strong}
\end{figure}

==> sections/biasedEQ1.tex <==
\section{Biased \EQ{1} Allocations}

In this section, we discuss the existence and computation of $i$-Biased \EQ{1} allocations. Recall that in an $i$-Biased \EQ{1} allocation $A$, agent $i$ is one of the richest agents, that is, $v_i(A_i) \geq v_j(A_j) ~\forall~j \neq i$.

\begin{comment}
\begin{theorem}
\label{thm:binary}
    Given a fair division instance with $n$ agents, $m$ items, and binary valuations, an $i$-Biased \EQ{1} allocation for any $i \in [n]$ always exists and can be computed in polynomial time.
\end{theorem}

\input{figures/algo_biasedbinary.tex}

\begin{proof}
Consider an \EQ{1} allocation $A$. If $v_i(A_i) \geq v_j(A_j) ~\forall~j \neq i$, then $A$ is an $i$-Biased \EQ{1} allocation and we are done. Otherwise, we show that the allocation $A'$ returned by \Cref{alg:biasedbinary} by modifying $A$ is $i$-Biased \EQ{1} Allocation. If agent $i$ values any good $g$ in any rich agent's bundle $A_r$, then it is reallocated to $i$. This implies that $v_i(A_i') = u+1$, $v_r(A_r') = u$, and everyone else's utility, which remains the same, is at most $u+1$. Therefore, $i$ is a rich agent under $A'$, hence $A'$ is an $i$-Biased \EQ{1} allocation. 

Suppose agent $i$ does not value anything owned by all the rich agents together, then one valuable good from each of the rich agents' bundles is wastefully allocated to $i$. We get, $v_i(A_i') = v_i(A_i) = u$, but for any rich agent $r$, we get $v_r(A_r') = v_r(A_r) - v_r(g) = v_r(A_r) - 1 = u$ and $v_j(A'_j) = v_j(A_j) = u ~\forall~j \in [n] \setminus \{i \cup R\}$. Therefore, $A'$ is an \EQ{} allocation and consequently an $i$-Biased \EQ{1} allocation.
\end{proof}
\end{comment}


